SAVER: Safe Learning-Based Controller for Real-Time Voltage Regulation

Fast and safe voltage regulation algorithms can serve as fundamental schemes for achieving a high level of renewable penetration in the modern distribution power grids. Faced with uncertain or even unknown distribution grid models and fast-changing power injections, model-free deep reinforcement learning (DRL) algorithms have been proposed to find the reactive power injections for inverters while optimizing the voltage profiles. However, such data-driven controllers can not guarantee satisfaction of the hard operational constraints, such as maintaining voltage profiles within a certain range of the nominal value. To this end, we propose SAVER: SAfe VoltagE Regulator, which is composed of an RL learner and a specifically designed, computational efficient safety projection layer. SAVER provides a plug-and-play interface for a set of DRL algorithms that guarantees the system voltages to be within safe bounds. Numerical simulations on real-world data validate the performance of the proposed algorithm.

==> other_idea.tex <==
% \textcolor{red}{Some possible methods:}
% \begin{itemize}
%     \item Solve (5) using optimization; if model is unknown, fit $\hat{R}, \hat{X}$ from data and use it as constraint with safety range $[\underline{v} - \xi, \overline{v} - \xi]$
%     \item Incorporate (5) as a safe layer using OptNet or some smarter ways that don't need solving the optimization
%     \item Learn constraint ICNN and solve projection with the ICNN constraint 
% \end{itemize}

% We can write out the Lagrangian as 
% \begin{equation}
%     L=\frac{1}{2}||\boldsymbol{q}-\boldsymbol{\pi}_\theta||^2_2+\bar{\boldsymbol{\lambda}}^T(\boldsymbol{Rp}+\boldsymbol{Xq}-\boldsymbol{\bar{v}})+\underline{\boldsymbol{\lambda}}^T(\boldsymbol{\underline{v}}-\boldsymbol{Rp}-\boldsymbol{Xq})
% \end{equation}

% We have the KKT conditions for the system as 

% \begin{equation}
%     \nabla_{\boldsymbol{q}} L=\boldsymbol{q}^*-\boldsymbol{\pi}_\theta+\boldsymbol{X}^T(\bar{\boldsymbol{\lambda}}-\underline{\boldsymbol{\lambda}})=\mathbf{0}
% \end{equation}

% \begin{equation}
%     \boldsymbol{\bar{\lambda}}^T(\boldsymbol{Rp}+\boldsymbol{Xq}-\boldsymbol{\bar{v}})=\boldsymbol{0};\quad \underline{\boldsymbol{\lambda}}^T(\boldsymbol{\underline{v}}-\boldsymbol{Rp}-\boldsymbol{Xq})=\boldsymbol{0}
% \end{equation}

% We have the following additional information:
% $\bar{\lambda_i}\geq 0;\quad  \underline{\lambda_i}\geq 0;$


% 1. have $\pi_\theta$

% 2. Evaluate $Rp+X\pi-v$

% don't know the rewards; interpret the policy safe/unsafe. 

% Multiple reward items that overwhelm the safety terms; no breakdown of the reward signal, very limited knowledge about voltage violation. 

% Realistic reward, optimize multiple aspects of power systems.

% Use multi parametric programming for this?

